Flow: Separating Consensus and Compute

Throughput limitations of existing blockchain architectures are one of the most significant hurdles for their wide-spread adoption. Attempts to address this challenge include layer-2 solutions, such as Bitcoin's Lightning or Ethereum's Plasma network, that move work off the main chain. Another prominent technique is sharding, i.e., breaking the network into many interconnected networks. However, these scaling approaches significantly increase the complexity of the programming model by breaking ACID guarantees increasing the cost and time for application development. In this paper, we describe a novel approach where we split the work traditionally assigned to cryptocurrency miners into two different node roles. Specifically, the selection and ordering of transactions are performed independently from their execution. The focus of this paper is to formalize the split of consensus and computation, and prove that this approach increases throughput without compromising security. In contrast to most existing proposals, our approach achieves scaling via separation of concerns, i.e., better utilization of network resources, rather than sharding. This approach allows established programming paradigms for smart contracts (which generally assume transactional atomicity) to persist without introducing additional complexity. We present simulations on a proof-of-concept network of 32 globally distributed nodes. While the consensus algorithm was identical in all simulations (a 2-step-commit protocol with rotating block proposer), block computation was either included in a consensus nodes' regular operations (conventional architecture) or delegated to specialized execution nodes (separation of concerns). Separation of concerns enables our system to achieve a throughput increase by a factor of 56 compared to conventional architectures without loss of safety or decentralization.

==> Makefile <==
TEX = pdflatex
BIB = bibtex

all : consensus_vs_compute.pdf

consensus_vs_compute.pdf: introduction.tex background.tex consensus_vs_compute.tex \
		consensus_vs_compute.bbl further_work.tex performance_modelling.tex \
		protocol.tex theoretical_motivation.tex
	$(TEX) consensus_vs_compute.tex

consensus_vs_compute.bbl: consensus_vs_compute.tex consensus_vs_compute.bib
	$(BIB) consensus_vs_compute.aux

clean:
	rm -f *.out *aux  *blg *log *toc *.ptb *.tod *.fls *.fdb_latexmk *.lof *.synctex.gz *.thm consensus_vs_compute.pdf

